Manifold Density Estimation via Generalized Dequantization

Density estimation is an important technique for characterizing distributions given observations. Much existing research on density estimation has focused on cases wherein the data lies in a Euclidean space. However, some kinds of data are not well-modeled by supposing that their underlying geometry is Euclidean. Instead, it can be useful to model such data as lying on a {\it manifold} with some known structure. For instance, some kinds of data may be known to lie on the surface of a sphere. We study the problem of estimating densities on manifolds. We propose a method, inspired by the literature on "dequantization," which we interpret through the lens of a coordinate transformation of an ambient Euclidean space and a smooth manifold of interest. Using methods from normalizing flows, we apply this method to the dequantization of smooth manifold structures in order to model densities on the sphere, tori, and the orthogonal group.

==> Manifold Density Estimation via Generalized Dequantization/algorithms/dequantization.tex <==
\begin{algorithm}[t!]
\caption{Training loop for dequantization inference. The target density $\pi_{\mathcal{Y}}$ is only relevant insofar as we must have samples available from it. The algorithm produces $\theta$ and $\phi$ that parameterize a distribution on $\R^m$ and a dequantization density on $\mathcal{Z}$. Together, these two densities can be combined to compute an estimate of the density using the right-hand side of \cref{eq:marginal-importance-sample-euclidean}.}
\label{alg:dequantization}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Samples from target density $\mathcal{D} \defeq (y_{1}, \ldots, y_{B})$ on an embedded manifold $\mathcal{Y}\subset\R^m$, step-size $\epsilon\in\R_+$.
\STATE Identify a smooth change-of-variables $G:\R^m\to \mathcal{Y}\times\mathcal{Z}$ where $\mathcal{Z}\subset \R^p$ is an auxiliary structure.
\STATE Let $\pi_{\R^m}$ be a density on $\R^m$ that is smoothly parameterized by $\theta\in \R^{n_\mathrm{amb}}$.
\STATE Let $\tilde{\pi}_{\mathcal{Z}}$ be a density on $\mathcal{Z}$ that is continuously parameterized by $y\in\mathcal{Y}$ and smoothly parameterized by $\phi\in \R^{n_{\mathrm{deq}}}$.
\WHILE {Not Done}
\STATE Use \cref{eq:evidence-lower-bound} or \cref{eq:log-likelihood} to compute an average loss over $\mathcal{D}$:
\begin{align}
    \mathcal{L}(\theta,\phi\vert \mathcal{D}) = \underset{y\sim\mathrm{Unif}(\mathcal{D})}{\mathbb{E}} \mathcal{F}(y \vert\theta,\phi)
\end{align}
where $\mathcal{F}$ is the right-hand side of \cref{eq:evidence-lower-bound} or \cref{eq:log-likelihood}, respectively.
\STATE Update $\theta = \theta + \epsilon \nabla_{\theta} \mathcal{L}(\theta,\phi\vert \mathcal{D})$ and $\phi = \phi + \epsilon \nabla_{\phi} \mathcal{L}(\theta,\phi\vert \mathcal{D})$.
\ENDWHILE
\STATE \textbf{Output}: Parameterized densities $\pi_{\R^m}(\cdot\vert \theta)$ and $\tilde{\pi}_{\mathcal{Z}}(\cdot\vert y,\phi)$ that can be used to perform density estimation on $\mathcal{Y}$ using \cref{eq:marginal-importance-sample-euclidean}.
\end{algorithmic}
\end{algorithm}

==> Manifold Density Estimation via Generalized Dequantization/appendices/embedded-manifolds.tex <==
\clearpage
\section{Embedded Manifolds}\label{app:embedded-manifolds}

A smooth manifold $\mathcal{X}$ of dimension $k$ is a second-countable Hausdorff space such that for every $x\in \mathcal{X}$ there is a homeomorphism between a neighborhood of $x$ and $\R^k$. By the Whitney Embedding Theorem (see, inter alia, \citep{lee2003introduction}), every smooth manifold can be smoothly embedded into Euclidean space of dimension $2k$. It is frequently possible to express an embedded manifold as the zero level-set of a constraint function: Let $g : \R^m\to\R^k$ be a smooth function and define $\mathcal{X}\defeq \set{x\in\R^m : g(x) = 0}$. If $\nabla g(x)\in\R^{k\times m}$ is a matrix of full-rank for every $x\in\mathcal{X}$, we say that $\mathcal{X}$ is an embedded manifold of rank $k$. 
To see how these definitions apply, let us consider some examples.

\subsection{Hypersphere}

The sphere in $\R^3$ is the zero level-set of the constraint function $g(x) \defeq x^\top x - 1$.

\subsection{Torus}

The torus is the preimage of the constraint function $g : \R^4\to\R^2$ defined by
\begin{align}
    g(x) \defeq \begin{pmatrix}
    x_1^2 + x_2^2 - 1 \\
    x_3^2 + x_4^2 - 1
    \end{pmatrix}.
\end{align}

\subsection{Stiefel Manifold}

A constraint function for the $\mathrm{Stiefel}(n, p)$ manifold is $g:\R^{n\times p} \to \R^{n\times n}$ defined by $g(\mathbf{M}) = \mathbf{M}^\top \mathbf{M} -\mathrm{Id}_n$. Using the $\mathrm{vec} : \R^{m\times n} \to\R^{mn}$ isomorphism, $\mathrm{Stiefel}(n, p)$ may also be embedded into $\R^{np}$.

==> Manifold Density Estimation via Generalized Dequantization/appendices/experimental-details.tex <==
\newpage
\section{Experimental Details}\label{app:experimental-details}


Here we include additional information about our experimental design.

\subsection{Sphere}

We consider the following unnormalized density on $\mathbb{S}^2$ given by
\begin{align}
    \pi_{\mathbb{S}^2}(y) \propto \sum_{i=1}^4 \exp(10y^\top \mu_i)
\end{align}
where $\mu_1 = (0.763, 0.643, 0.071)$, $\mu_2= ( 0.455, -0.708 ,  0.540)$, $\mu_3 = (0.396, 0.271, 0.878)$, and $\mu_4 = (-0.579 ,  0.488, -0.654)$. 

When using RealNVP, the total number of learnable parameters in our dequantization model is $5,894$; dequantization with an ambient ODE has $5,705$ learnable parameters; in the case of the M\"{o}bius transform the total number of learnable parameters is $5,943$; for the manifold ODE implementation, we have $5,533$ parameters.

On $\mathbb{S}^3$, we consider an unnormalized density proportional to
\begin{align}
    \pi_{\mathbb{S}^3}(y) &\propto \sum_{i=1}^4 \exp(10y^\top \mu_i) \\
    \mu_1&=(-0.129,  0.070,  0.659, -0.738) \\
    \mu_2&=(-0.990 , -0.076,  0.118, -0.017) \\
    \mu_3&=(0.825 , -0.484 ,  0.061,  0.285) \\
    \mu_4&=(-0.801 ,  0.592 , -0.024,  0.081).
\end{align}

When using RealNVP, the total number of learnable parameters in our dequantization model is $21,854$; dequantization with an ambient ODE has $21,386$ learnable parameters; in the case of the M\"{o}bius transform the total number of learnable parameters is $25,406$; for the manifold ODE implementation, we have $21,204$ parameters. For dequantization we use 100 samples per batch and use rejection sampling to draw samples from the unnormalized target density at each iteration.

\subsection{Torus}

Expressed in terms of their {\it angular} coordinates (as opposed to their embedding into $\R^4$), the densities on the torus are as follows:
\begin{description}
\item[Unimodal] $\pi^{\mathrm{uni}}_{\mathbb{T}^2}(\theta_1,\theta_2\vert\phi) \propto \exp(\cos(\theta_1 - \phi_1) + \cos(\theta_2 - \phi_2))$ with $\phi=(4.18,5.96)$.
\item[Multimodal] $\pi_{\mathbb{T}^2}^\mathrm{mul}(\theta_1,\theta_2) \propto\sum_{i=1}^3 \pi_{\mathbb{T}^2}^\mathrm{uni}(\theta_1,\theta_2\vert \phi_i)$ where $\phi_1=(0.21,2.85)$, $\phi_2=(1.89,6.18)$, and $\phi_3=(3.77,1.56)$.
\item[Correlated] $\pi_{\mathbb{T}^2}^{\mathrm{cor}}(\theta_1,\theta_2) \propto \exp(\cos(\theta_1+\theta_2-1.94))$.
\end{description}

The number of learnable parameters in the dequantization models is $6,106$; in the M\"{o}bius flow model, the number of learnable parameters is $5,540$; for the direct method, the number of learnable parameters is $5,406$. For dequantization we use 100 samples per batch and use rejection sampling to draw samples from the unnormalized target density at each iteration.

\subsection{Orthogonal Group}

Drawing inspiration from the orthogonal Procrustes problem, we define the unnormalized density by
\begin{align}
    \label{eq:procrustes-density}\pi_{\mathrm{O}(n)}(\mathbf{O}) \propto \exp\paren{-\frac{1}{2\sigma^2}\Vert \mathbf{B} - \mathbf{O}\mathbf{A}\Vert_\mathrm{fro}^2},
\end{align}
where $\mathbf{A},\mathbf{B}\in\R^{n\times p}$. Given samples from \cref{eq:procrustes-density}, we may apply our dequantization procedure to perform density estimation. In our experiments we take $p=10$ and $n=3$. For dequantization we use rejection sampling to draw samples from the posterior. Then, with these fixed samples, we use batches of 100 samples to train the ambient and dequantization distributions.

\subsection{Special Orthogonal Group}

Let $\mathbf{R}\in\R^{n\times n}$ be a reflection matrix and notice that $\set{\mathrm{SO}(n), \mathbf{R}\mathrm{SO}(n)}$ is partition of $\mathrm{O}(n)$. Given a density on $\R^{n\times n}$, using the methods described in \cref{subsec:stiefel-manifold}, we may obtain a density on $\mathrm{O}(n)$. Then, we define the function $S:\mathrm{O}(n)\to\mathrm{SO}(n)$ by
\begin{align}
    S(\mathbf{O}) \defeq \begin{cases}
    \mathbf{O} & ~\text{if}~ \mathrm{det}(\mathbf{O}) = +1 \\
    \mathbf{R}\mathbf{O} & ~\text{if}~ \mathrm{det}(\mathbf{O}) = -1
    \end{cases},
\end{align}
where $\mathbf{R}$ is a reflection matrix. Now, define $S_1(\mathbf{O}) \defeq \mathbf{O}$ and $S_2(\mathbf{O}) \defeq \mathbf{R}\mathbf{O}$, which satisfy $S_1 = S\vert \mathrm{SO}(n)$ and $S_2 = S\vert \mathbf{R}\mathrm{SO}(n)$. Both $S_1$ and $S_2$ are self-inverse and volume-preserving maps on their respective domains so we may obtain a density on $\mathrm{SO}(n)$ as
\begin{align}
    \label{eq:son-likelihood} \pi_{\mathrm{SO}(n)}(\mathbf{O}) = \pi_{\mathrm{O}(n)}(\mathbf{O}) + \pi_{\mathrm{O}(n)}(\mathbf{R}\mathbf{O}).
\end{align}
One may immediately seek to minimize the negative log-likelihood of data using \cref{eq:son-likelihood}. Alternatively, we use the following ELBO in our our experiments:
\begin{align}
    \log \pi_{\mathrm{SO}(n)}(\mathbf{O}) &\geq \underset{\mathbf{S}\sim\mathrm{Unif}(\mathrm{Id}_n, \mathbf{R})}{\mathbb{E}}  \underset{\mathbf{L}\sim \tilde{\pi}_{\mathrm{Tri}_+}}{\mathbb{E}} \frac{\pi_{\R^{n\times n}}(\mathbf{S}\mathbf{O}\mathbf{P})}{\mathrm{det}(\nabla G(\mathbf{S}\mathbf{O}\mathbf{P}))\cdot \tilde{\pi}_{\mathrm{Tri}_+}(\mathbf{L})},
\end{align}
where, as in \cref{ex:stiefel-dequantization}, $\mathbf{P} =\mathbf{L}\mathbf{L}^\top$. For a short derivation of this ELBO, see \cref{app:son-elbo}.

We consider the following multimodal density on $\mathrm{SO}(3)$:
\begin{align}
    \pi_{\mathrm{SO}(3)}(\mathbf{O}) \propto \sum_{i=1}^3 \exp(-\frac{1}{2\sigma^2} \Vert \mathbf{O} - \Omega_i\Vert_\text{fro}^2)
\end{align}
where in our experiments we set $\sigma=1/2$, $\Omega_1=\mathrm{diag}(1, 1, 1)$, $\Omega_2=\mathrm{diag}(-1, -1, 1)$, and $\Omega_3=\mathrm{diag}(-1, 1, -1)$. For dequantization we use rejection sampling to draw samples from the posterior. Then, with these fixed samples, we use batches of 100 samples to train the ambient and dequantization distributions.


==> Manifold Density Estimation via Generalized Dequantization/appendices/integer-dequantization.tex <==
\clearpage
\section{Dequantizing the Integers}\label{app:integer-dequantization}

We now consider how to apply \cref{cor:partition-change-of-variables,thm:manifold-change-of-variables} to the dequantization of integers and draw a connection to dequantization in normalizing flows \citep{hoogeboom2020learning}. Let $\pi_{\mathbb{R}}$ be a probability density on $\R$. Consider the function $T:\R\to\mathbb{Z}\times[0, 1)$ defined by $T(x) = (\lfloor x\rfloor, x - \lfloor x\rfloor)$. Consider the partition of $\R$ given by $\mathcal{O}_n = [n, n+1)$; on each $\mathcal{O}_n$ we have that $T_n(x) \defeq (n, x-n)$ satisfies $T_n=T\vert \mathcal{O}_n$; moreover, on each $\mathcal{O}_n$, the transformation $T_n$ is invertible (the inverse map is $(n, r)\mapsto n+r$) and preserves volume, which implies a unit Jacobian determinant. Therefore, the associated density on $\mathbb{Z}\times [0, 1)$ is given by $\pi_{\mathbb{Z}\times [0, 1)}(n, r) = \pi_{\R}(n+r)$. We may view $\mathbb{Z}\times[0, 1)$ as a coordinate system for $\R$. If we wish to integrate out the nuisance variables in the unit interval, we obtain the marginal density on $\mathbb{Z}$ as
\begin{align}
    \pi_\mathbb{Z}(n) = \int_0^1 \pi_{\R}(n+r) ~\mathrm{d}r.
\end{align}
By choosing $\tilde{\pi}_{[0,1)}$ as, for example, a Uniform distribution, one obtains the traditional uniform dequantization.
Choosing a more complex distribution, for example, a Beta distribution (with parameters possibly depending on $n$) one obtains an importance sampling formula for the marginal density as $\pi_{\mathbb{Z}}(n) = \underset{r\sim \tilde{\pi}_{[0,1)}(r)}{\mathbb{E}} \frac{\pi_\R(n+r)}{\tilde{\pi}_{[0,1)}(r)}$.
This can be optimized through a variational bound, giving variational dequantization \citep{ho2019flow}.
Optimizing it directing gives importance weighted dequantization \citep{hoogeboom2020learning}.


==> Manifold Density Estimation via Generalized Dequantization/appendices/metrics.tex <==
\newpage
\section{Evaluation Metrics}\label{app:evaluation-metrics}

Given a density $\pi_\mathcal{Y}(y) \propto \exp(-u(y))$, known up to proportionality, we consider several performance metrics for the dequantization method we propose.
The error of the first order moment is defined by, 
\begin{align}
\Vert\underset{y\sim\pi_\mathcal{Y}}{\mathbb{E}}\left[y\right] - \underset{\hat{y}\sim\hat{\pi}_{\mathcal{Y}}}{\mathbb{E}}\left[\hat{y}\right]\Vert_2.
\end{align}
The error of the second (centered) moment is defined by 
\begin{align}
\Vert \underset{y\sim\pi_\mathcal{Y}}{\mathrm{Cov}}\left(y\right) - \underset{\hat{y}\sim\hat{\pi}_{\mathcal{Y}}}{\mathrm{Cov}}\left(\hat{y}\right)\Vert_\mathrm{fro}.
\end{align}

The Kullback-Leibler divergence of $\hat{\pi}_\mathcal{Y}$ and $\pi_\mathcal{Y}$ is
\begin{align}
    \mathrm{KL}(\hat{\pi}_{\mathcal{Y}}\Vert \pi_\mathcal{Y}) &\defeq \underset{\hat{y}\sim\hat{\pi}_{\mathcal{Y}}}{\mathbb{E}} \log \frac{\hat{\pi}_{\mathcal{Y}}(\hat{y})}{\pi_\mathcal{Y}(\hat{y})} \\
    &= \underset{\hat{y}\sim\hat{\pi}_{\mathcal{Y}}}{\mathbb{E}}\left[ \log \hat{\pi}_{\mathcal{Y}}(\hat{y}) + u(\hat{y})\right] + \log Z,
\end{align}
where $Z$ is the normalizing constant of $\pi_\mathcal{Y}(y)$. We can estimate $Z$ via importance sampling according to
\begin{align}
    Z = \underset{\hat{y}\sim\hat{\pi}_{\mathcal{Y}}}{\mathbb{E}}\left[\frac{\exp(-u(\hat{y})))}{\hat{\pi}_{\mathcal{Y}}(\hat{y})}\right],
\end{align}
which permits us to compute a Monte Carlo estimate of the Kullback-Leibler divergence. The reverse direction of the KL-divergence $\mathrm{KL}(\pi_\mathcal{Y}\Vert \hat{\pi}_\mathcal{Y})$ may be similarly computed.

Let $\set{\hat{y}_1,\ldots,\hat{y}_n}$ be a collection of independent identically-distributed  samples from $\hat{\pi}_{\mathcal{Y}}$. The number of effective independent samples is the quantity,
\begin{align}
    \mathrm{ESS} \defeq \frac{\paren{\sum_{i=1}^n \omega_i}^2}{\sum_{i=1}^n \omega_i^2}
\end{align}
where $\omega_i = \exp(-u(\hat{y}_i)) / \hat{\pi}_{\mathcal{Y}}(\hat{y}_i)$. See \citep{10.5555/1571802,doucet2001sequential} for details on the ESS metric. Following \citep{DBLP:journals/corr/abs-2002-02428}, we report the relative ESS, which the ratio of the effective sample size and $n$, the number of samples. When a Monte Carlo approximation of the evaluation metric is required, we use rejection sampling in order to obtain samples from the density $\pi_\mathcal{Y}$.

==> Manifold Density Estimation via Generalized Dequantization/appendices/overview-of-normalizing-flows.tex <==
\clearpage
\section{Overview of Normalizing Flows}

This section describes the Euclidean normalizing flows used in this paper.

\subsection{RealNVP}

Let $x\in\R^m$ and let $n,p\in\mathbb{N}$ satisfy $m=n+p$. Consider partitioning $x$ into components $x_a\in\R^n$ and $x_b\in\R^p$ by taking the first $n$ and last $p$ components from $x$, respectively. Let $\mu(\cdot;\theta) :\R^n\to \R^p$ and $\sigma : \R^n\to\R^p_+$ be a functions parameterized by $\theta\in\R^{d_\mu}$ and $\phi\in\R^{d_{\sigma}}$, respectively. Compute the affine transformation of $x_b$ according to
\begin{align}
    y_b \defeq \sigma(x_a) \odot x_b + \mu(x_a) \\
    y \defeq (x_a, y_b).
\end{align}
The transformation $x \mapsto y$ has a Jacobian of the form,
\begin{align}
    \nabla_x y = \begin{pmatrix} \mathrm{Id}_n & \mathbf{0}_{n\times p} \\ \nabla_{x_a} y_b & \mathrm{diag}(\sigma(x_a)) \end{pmatrix}.
\end{align}
The key observation about this Jacobian is that it has a lower-triangular structure. Therefore, its determinant is the product of its diagonal elements.

The transformation $x\mapsto y$ is also invertible. Let $(y_a, y_b)$ be the corresponding partition of $y$. The inverse map is given by,
\begin{align}
    x_b = (y_b - \mu(y_a)) \oslash \sigma(y_a) \\
    x_a = y_a.
\end{align}

With the inverse and Jacobian determinant available, we may apply the transformation $x\mapsto y$ in the Euclidean change-of-variables formula. This transformation is called RealNVP. In practice, it is common to chain multiple RealNVP transformations together in order to obtain a more expressive flow. One may also permute the elements of $y$ after each application of the RealNVP transformation (which is, of course, an invertible, volume-preserving transformation) in order to construct affine transformations of different variables.

\subsection{Neural ODE}

Let $x\in\R^m$ and let $f(\cdot, \cdot; \theta) : \R^m\times \R\to\R^m$ be a smooth function parameterized by $\theta\in\R^d$. Consider solving the initial value problem defined by,
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} \phi_t(x) &= f(\phi_t(x), t; \theta) \\
    \phi_0(x) &= x.
\end{align}
The map $\phi_{(\cdot)}(\cdot) : \R\times\R_m\to\R_m$ is called the flow of $f$. The existence and uniqueness of differential equations leads to the group property of flows:
\begin{align}
    \phi_{t+s}(x) = \phi_t(\phi_s(x)).
\end{align}
In particular, since $\phi_0(x)=x$, we have $\phi_{-t}\circ \phi_t = \mathrm{Id}$ or $\phi_t^{-1} = \phi_{-t}$ so that the inverse flow map is obtained from the flow map with a negated time index.

How does the flow of a vector field affect probability? This is an important question that can be answered at varying levels of sophistication. One elegant analysis uses techniques from fluid mechanics and the Lie derivative theorem. In the following we adopt a simpler, if more mechanical, derivation of the rate of change of the Jacobian determinant.
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} \mathrm{det}(\nabla_x \phi_t(x)) &= \mathrm{det}(\nabla_x \phi_t(x)) ~\mathrm{trace}\paren{\left[\nabla_x \phi_t(x)\right]^{-1} \frac{\mathrm{d}}{\mathrm{d}t} \nabla_x\phi_t(x)} \\
    &= \mathrm{det}(\nabla_x \phi_t(x)) ~\mathrm{trace}\paren{\left[\nabla_x \phi_t(x)\right]^{-1} \mathbf{D}_x f(\phi_t(x), t; \theta)} \\
    &= \mathrm{det}(\nabla_x \phi_t(x)) ~\mathrm{trace}\paren{\left[\nabla_x \phi_t(x)\right]^{-1} \nabla_x f(\phi_t(x), t; \theta) \nabla_x \phi_t(x)} \\
    &= \mathrm{det}(\nabla_x \phi_t(x)) ~\mathrm{trace}\paren{\nabla_x f(\phi_t(x), t; \theta)} \\
    &= \mathrm{det}(\nabla_x \phi_t(x)) ~\mathrm{div}(f(\phi_t(x), t; \theta))
\end{align}
From which it follows that,
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} \log\abs{\mathrm{det}(\nabla_x \phi_t(x))} = \mathrm{div}(f(\phi_t(x), t; \theta)).
\end{align}
Let $\pi :\R^m\to\R_+$ be a probability density and let $x\sim\pi$. Let $\pi_t(\phi_t(x))$ be the density of $\phi_t(x)$. Because $\log \pi_t(\phi_t(x)) = \log \pi(x) - \log\abs{\mathrm{det}(\nabla_x \phi_t(x))}$, we have,
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} \log \pi_t(\phi_t(x)) = -\mathrm{div}(f(\phi_t(x), t; \theta)).
\end{align}
This formula is sometimes called the {\it instantaneous change-of-variables formula}. From the initial condition $\phi_0(x) = x$, we obtain that $\log\abs{\mathrm{det}(\nabla_x \phi_0(x))} = 0$, which gives an initial condition for the time evolution of the Jacobian determinant.

In general, none of the initial value problems described so far have analytical solutions. This necessitates the use of numerical integrators to compute the map $\phi_t(\cdot)$, its inverse, and the Jacobian determinant correction from the instantaneous change-of-variables formula. The method is called {\it neural ODE} because $f(\cdot, \cdot;\theta)$ is often chosen to be a neural network parameterized by $\theta$.



==> Manifold Density Estimation via Generalized Dequantization/appendices/polar-decomposition.tex <==
\clearpage
\section{Polar Decomposition Isomorphism}\label{app:polar-decomposition-isomorphism}

\begin{proposition}
Let $\mathbf{A}$ be a real, positive semi-definite matrix. Then there exists a unique real, positive semi-definite matrix $\mathbf{B}$ such that $\mathbf{A} = \mathbf{B}\mathbf{B}$. We call $\mathbf{B}$ the principal square root of $\mathbf{A}$ and may write $\mathbf{B}=\sqrt{\mathbf{A}}$.
\end{proposition}
\begin{definition}[Stiefel Manifold]
The $\mathrm{Stiefel}(m, n)$ manifold is the subset of $\R^{m\times n}$ of orthogonal matrices. That is,
\begin{align}
    \mathrm{Stiefel}(m, n) = \set{\mathbf{X} \in\R^{m\times n} : \mathbf{X}^\top\mathbf{X} = \mathrm{Id}}
\end{align}
\end{definition}
\begin{definition}
The set of $n\times n$ positive-definite matrices is denoted $\mathrm{PD}(n)$.
\end{definition}
\begin{definition}[Non-Square Polar Decomposition]
Let $\mathbf{A}\in\R^{m\times n}$ with $m\geq n$ have the (thin) singular value decomposition $\mathbf{A} = \mathbf{U}\Sigma\mathbf{V}^\top$ where $\mathbf{U}\in \mathrm{Stiefel}(m, n)$ and $\mathbf{V}^\top \in \mathrm{O}(n)$. Then we define the non-square polar decomposition to be $\mathbf{A} = \mathbf{O}\mathbf{P}$ where,
\begin{align}
    \label{eq:polar-stiefel} \mathbf{O} &\defeq \mathbf{U}\mathbf{V}^\top \\
    \label{eq:polar-psd} \mathbf{P} &\defeq \mathbf{V}\Sigma\mathbf{V}^\top.
\end{align}
\end{definition}
\begin{lemma}
The quantity $\mathbf{P}$ in \cref{eq:polar-psd} is uniquely defined.
\end{lemma}
\begin{proof}
The strategy is to show that $\mathbf{P}$ is the unique principal square root of a positive semi-definite matrix. It is immediately clear from the definition that $\mathbf{P}$ is itself positive semi-definite. Consider the positive semi-definite matrix
\begin{align}
    \mathbf{A}^\top\mathbf{A} &= (\mathbf{V}\Sigma\mathbf{U}^\top) (\mathbf{U}\Sigma\mathbf{V}^\top) \\
    &= \mathbf{V}\Sigma\Sigma\mathbf{V}^\top \\
    &= (\mathbf{V}\Sigma\mathbf{V}^\top)(\mathbf{V}\Sigma\mathbf{V}^\top) \\
    &=\mathbf{P}\mathbf{P}.
\end{align}
By identification $\mathbf{P}$ is the principal square root of $\mathbf{A}^\top\mathbf{A}$ so it is unique.
\end{proof}
\begin{proposition}
Let $\Sigma = \text{diag}(\sigma_1,\ldots,\sigma_n)$ and suppose that $\sigma_1\geq \sigma_2\geq\ldots\geq \sigma_n > 0$. Then, the quantity $\mathbf{O}$ in \cref{eq:polar-stiefel} is uniquely defined.
\end{proposition}
\begin{proof}
If $\sigma_n > 0$ then 
\begin{align}
    \text{det}(\mathbf{P}) &= \text{det}(\mathbf{V}) \cdot\text{det}(\Sigma) \cdot\text{det}(\mathbf{V}^\top) \\
    &= \prod_{i=1}^n \sigma_i \\
    &> 0.
\end{align}
Thus, $\mathbf{P}$ is invertible. Thus, $\mathbf{O} = \mathbf{A}\mathbf{P}^{-1}$.
\end{proof}
Note that the condition on the singular values is equivalent to the statement that $\mathbf{A}$ has full-rank.
\begin{lemma}
If $\mathbf{A}$ has full-rank then $\mathbf{P}\in\mathrm{PD}(n)$.
\end{lemma}
\begin{proof}
If $\mathbf{A}$ has full-rank then all the singular values are strictly positive. Thus, $\mathbf{V}\Sigma\mathbf{V}^\top$ is an eigen-decomposition of $\mathbf{P}$ whose eigenvalues are all positive. Since a matrix is positive-definite if and only if all of its eigenvalues are positive, we conclude that $\mathbf{P}\in\mathrm{PD}(n)$.
\end{proof}
\begin{lemma}
The quantity $\mathbf{O}$ in \cref{eq:polar-stiefel} is an element of $\mathrm{Stiefel}(m, n)$.
\end{lemma}
\begin{proof}
\begin{align}
    \mathbf{O}^\top\mathbf{O} &= \mathbf{V}\mathbf{U}^\top\mathbf{U}\mathbf{V}^\top \\
    &= \mathbf{V}\mathbf{V}^\top \\
    &= \mathrm{Id}.
\end{align}
\end{proof}

\begin{proposition}
Given $\mathbf{O}\in\mathrm{Stiefel}(m, n)$ and $\mathbf{P}\in\mathrm{PD}(n)$, we may always write $\mathbf{O}$ and $\mathbf{P}$ in the form of \cref{eq:polar-stiefel,eq:polar-psd}.
\end{proposition}
\begin{proof}
Since $\mathbf{P}\in\mathrm{PD}(n)$, by the spectral theorem there exists an orthonormal basis $\set{v_1,\ldots,v_n}$ of $\R^n$ and real, positive eigenvalues $\lambda_1,\ldots,\lambda_n$, such that $\mathbf{P} = \mathbf{V}\Sigma\mathbf{V}^{-1} = \mathbf{V}\Sigma\mathbf{V}^\top$ where $\mathbf{V}\in \R^{n\times n}$ is the collection of $\set{v_1,\ldots,v_n}$ as columns and $\Sigma=\mathrm{diag}(\lambda_1,\ldots,\lambda_n)$. 

Using this $\mathbf{V}$ we may compute $\mathbf{U} = \mathbf{O}\mathbf{V}$, which is an orthogonal matrix:
\begin{align}
    \mathbf{U}^\top \mathbf{U} &= \mathbf{V}^\top\mathbf{O}^\top\mathbf{O}\mathbf{V} \\
    &= \mathbf{V}^\top\mathbf{V} \\
    &= \mathrm{Id}.
\end{align}
Define the matrix $\mathbf{A}=\mathbf{O}\mathbf{P}$. By inspection, a (thin) singular value decomposition of $\mathbf{A}$ is
\begin{align}
    \mathbf{A} &= \mathbf{U}\Sigma\mathbf{V}^\top
\end{align}
since
\begin{align}
    \mathbf{O}\mathbf{P} &= \mathbf{U}\mathbf{V}^\top \mathbf{V}\Sigma\mathbf{V}^\top \\
    &= \mathbf{U}\Sigma\mathbf{V}^\top.
\end{align}
Finally, $\mathbf{U}\in\mathrm{Stiefel}(m, n)$, $\Sigma$ has only positive entries, and $\mathbf{V}\in\mathrm{O}(n)$, which are the conditions of a thin singular value decomposition.
\end{proof}

==> Manifold Density Estimation via Generalized Dequantization/appendices/practical-considerations.tex <==
\newpage
\section{Practical Considerations}

\input{tables/elements}

\subsection{The Ambient Euclidean Space}

It is frequently the case that a manifold has a natural embedding into Euclidean space. For instance, the sphere $\mathbb{S}^{m-1}$ is naturally embedded into $\R^{m}$. The Stiefel manifold is a subset of $\R^{n\times p}$ satisfying an orthonormality condition; therefore, it is naturally embedded into $\R^{n\times p}$. For some manifolds, the choice may require some consideration. For instance, a torus $\mathbb{T}^2$ may be regarded as a product manifold of two circles, each of which are naturally embedded into $\R^2$ so that the entire torus is embedded into $\R^4$ (this is called the {\it Clifford torus}). An alternative is the familiar embedding of the torus as a ``doughnut'' in $\R^3$, although in this case it may be non-obvious how to construct a suitable mapping $G$ between $\R^3$, the doughnut torus, and some auxiliary choice of one-dimensional manifold.

\subsection{The Change-of-Variables and Auxiliary Manifold}

We have seen several examples wherein manifolds of interest appear alongside an auxiliary manifold when an ambient Euclidean space is transformed under a change-of-variables. In general, one would like to identify a transformation $G:\mathcal{X}\to\mathcal{Y}\times\mathcal{Z}$, satisfying the conditions of \cref{thm:manifold-change-of-variables} or \cref{cor:partition-change-of-variables}, such that it will be straightforward to formulate importance sampling random variables on $\mathcal{Z}$ so as to obtain the marginal density on $\mathcal{Y}$.

\subsection{Dequantization Density}

Dequantization densities $\tilde{\pi}_\mathcal{Z}$ on $\mathcal{Z}$ has to respect the constraints of the auxiliary manifold. For instance, if $\mathcal{Z}=\R_+$ we must choose a dequantization density whose support is the positive real numbers and which is non-vanishing. The requirement that $\tilde{\pi}_\mathcal{Z}$ be non-vanishing (that is, $\tilde{\pi}_\mathcal{Z}(z) > 0$ for all $z\in\mathcal{Z}$) is important so as to avoid division-by-zero singularities in the importance sampling formula \cref{eq:marginal-importance-sample-euclidean}. We have already seen some examples of dequantization densities that respect the constraints of the auxiliary manifold in \cref{sec:theory}. In each of these cases, the dequantization distribution is parameterized (for example, the Gamma distribution is parameterized by its shape and scale); it may be desirable to choose these parameters to depend on the location $y\in \mathcal{Y}$. To accomplish this, one may construct a neural network with parameters $\phi$ and input $y$ whose output is the parameterization of the dequantization distribution. Thus the dequantization distribution may be in general expressed as $\tilde{\phi}_\mathcal{Z}(\cdot\vert \phi, y)$.



==> Manifold Density Estimation via Generalized Dequantization/appendices/proof-manifold-change-of-variables.tex <==
\newpage
\section{Proof of Manifold Change-of-Variables Formula}

\begin{proposition}
Let $A\subseteq \R^m$ and let $G:A\to\R^n$ be a smooth function. Suppose $m<n$. Define the embedded manifold $M\defeq G(A)$. Let $\pi$ be a real-valued, continuous function on $M$. Then,
\begin{align}
    \int_{M} \pi(x) ~\mathrm{dVol}(x) = \int_{A} \pi(G(t)) \cdot \sqrt{\mathrm{det}((\nabla G(t))^\top (\nabla G(t)))} ~\mathrm{d}t
\end{align}
where $\mathrm{dVol}$ is the volume measure on $M$.
\end{proposition}
\begin{proof}
See \citep{frank-jones}.
\end{proof}
\begin{corollary}
Define,
\begin{align}
    \pi_{\R^m}(t) \defeq \pi(G(t)) \cdot \sqrt{\mathrm{det}((\nabla G(t))^\top (\nabla G(t)))}.
\end{align}
Then rearranging immediately implies,
\begin{align}
    \pi(G(t)) = \frac{\pi_{\R^m}(t)}{\sqrt{\mathrm{det}((\nabla G(t))^\top (\nabla G(t)))}},
\end{align}
which is the manifold change-of-variables formula. 
\end{corollary}


What follows now is a more detailed exposition on this result using Riemannian geometry.

Let $U$ be an open subset of $\R^m$.  Let $G$ be a continuous function from $U\to\R^n$ that is a homeomorphism on its image. That is, defining $\mathcal{M}\defeq \set{G(x) : x\in U}\subset \R^n$, we find that $G$ has a continuous inverse on $\mathcal{M}$. As a subset of $\R^n$, we can equip $\mathcal{M}$ with the subspace topology and find that $\mathcal{M}$ is a topological $m$-manifold. Under these assumptions, it immediately follows that $(\mathcal{M}, G^{-1})$ is a {\it global} coordinate chart in the sense of differential geometry.

If we further assume that $G$ and its inverse are smooth functions (in the sense of ordinary calculus), then it follows that $\mathcal{M}$ is globally diffeomorphic to $U$. Evidently, our discussion allows $m\leq n$. If the Jacobian (in the sense of ordinary calculus) of $G$, denoted $\nabla G : U\to\R^{n\times m}$, has the property that at every $x\in U$, $\mathrm{rank}(\nabla G(x)) = m$, then $G$ is called a smooth immersion; this is equivalent to $\nabla G$ having full-rank at each $x\in U$. Moreover, because $G$ is homeomorphic onto its image, $G$ is also a smooth embedding.

The tangent space of a smooth manifold can be constructed as the vector space of velocities that a particle moving along the manifold may exhibit at a point. Formally, let $(a,b)\subset \R$ be an open interval and let $x:(a, b)\to U$ be a parameterized smooth curve in $U$. The composition $y\defeq G\circ x : (a,b)\to\mathcal{M}$ is then a parameterized smooth curve on $\mathcal{M}$. The velocity of $y$ is then computed as,
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} y(t) = \frac{\mathrm{d}}{\mathrm{d}t} (G\circ x)(t) = \nabla G(x(t)) \dot{x}(t).
\end{align}
From the preceding discussion, $\nabla G(x(t)) \in \R^{n\times m}$ is a matrix of full-rank and therefore has $m$ linearly-independent $n$-dimensional columns. Since $\dot{x}(t)\in\R^m$ can be arbitrary, we find that the tangent space of $\mathcal{M}$ at $y(t)$ is the vector space spanned by the columns of $\nabla G(x(t))$; note that these basis vectors depend only on the position in $U$ and not on time. Given $y\in\mathcal{M}$, we denote the tangent space by $\mathrm{T}_{y}\mathcal{M} = \set{\nabla G(x) c : c\in\R^m, x = G^{-1}(y)}$ which is a vector subspace of $\R^n$. In the following, we make use of the common identification $\mathrm{T}_x\R^m\cong \R^m$.

A smooth manifold can be turned into a Riemannian manifold by equipping its tangent spaces with an inner product called the Riemannian metric. Formally, given $y\in\mathcal{M}$, $g(y) \mapsto \langle\cdot,\cdot\rangle_{y}$ where $\langle \cdot,\cdot\rangle_y : \mathrm{T}_y\mathcal{M}\times\mathrm{T}_y\mathcal{M}\to\R$ is an inner product. Given the discussion so far, there is no prescription for a Riemannian metric. However, we may ``prefer'' the Riemannian metric that is induced from the ambient Euclidean space $\R^n$. For $\tilde{y}\in\R^n$, the Euclidean metric is defined by $\langle u, v\rangle_{\tilde{y}} = u^\top v$ where $u,v\in\mathrm{T}_{\tilde{y}}\R^n \cong\R^n$. The induced metric on $\mathcal{M}\subset\R^n$ is then defined by $\langle u,v\rangle_y = u^\top v$ where $u$ and $v$ are viewed as vectors in $\R^n$ satisfying $u,v\in\mathrm{T}_{y}\mathcal{M}$.

Given a metric on $\mathcal{M}$, we can compute an associated metric on $U$ called the {\it  pullback metric}. The pullback metric is defined by,
\begin{align}
    \tilde{g}(x)(\tilde{u},\tilde{v}) &= g(G(x))(\nabla G(x)\tilde{u}, \nabla G(x)\tilde{v}) \\
    &= \tilde{u}^\top \nabla G(x)^\top \nabla G(x) \tilde{v}
\end{align}
where $\tilde{u},\tilde{v}\in \mathrm{T}_x\R^m\cong \R^m$. From the condition that $\nabla G(x)$ is a matrix of full-rank for each $x\in U$, it can be shown that $\nabla G(x)^\top \nabla G(x)$ is a positive definite matrix. Hence the pullback metric is a proper inner product. Unlike the induced metric on $\mathcal{M}$ which has no real dependency on $y\in\mathcal{M}$, the pullback metric does depend on $x\in U$ through $\nabla G(x)^\top \nabla G(x)$. The pullback metric can be regarded as the expression of the induced metric on $\mathcal{M}$ in the global coordinates of $U$. Indeed, if $y=G(x)$, recall that every $u\in \mathrm{T}_y\mathcal{M}$ can be expressed as $u=\nabla G(x)\tilde{u}$ where $\tilde{u}\in\R^m$; the unique $\tilde{u}$ can be computed from
\begin{align}
    \tilde{u} = (\nabla G(x)^\top\nabla G(x))^{-1} \nabla G(x)^\top u.
\end{align}



In our construction, we have described how to induce a metric on $\mathcal{M}$ via the Euclidean metric in the embedding space. We then described how the metric materializes in the global coordinate system via the pullback metric. We are now in a position to state how these objects inform integration on Riemannian manifolds. 
We have the following theorem.
\begin{theorem}
Let $\mathrm{dVol}$ denote the Riemannian volume element on $\mathcal{M}$ when the metric on $\mathcal{M}$ is the induced Euclidean metric from $\R^n$. Given a smooth function $f : \mathcal{M}\to\R$, its integral over $\mathcal{M}$ can be expressed in terms of the global coordinate system as,
\begin{align}
    \int_{\mathcal{M}} f(y) ~\mathrm{dVol}(y) = \int_{U} f(G(x)) \cdot \sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))} ~\mathrm{d}x.
\end{align}
\end{theorem}
A proof of this result may be found in \citep{frank-jones}. More sophisticated variants of this result may be found textbooks on differential geometry; see, {\it inter alia}, \citep{lee2003introduction}.

If $\pi_{\mathcal{M}}$ is a density on $\mathcal{M}$, $y\sim \pi_{\mathcal{M}}$ and $A\subset \mathcal{M}$, then we have,
\begin{align}
    \underset{y\sim \pi_{\mathcal{M}}}{\mathrm{Pr}}\left[y\in A\right] &= \int_{\mathcal{M}} \mathbf{1}\set{y \in A}\cdot \pi_{\mathcal{M}}(y)~\mathrm{dVol}(y) \\
    &= \int_U \pi_{\mathcal{M}}(G(x)) \cdot\mathbf{1}\set{G(x)\in A} \cdot\sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))} ~\mathrm{d}x \\
    &= \underset{x\sim \pi_{U}}{\mathrm{Pr}}\left[x\in G^{-1}(A)\right]
\end{align}
where
\begin{align}
    \pi_U(x) = \pi_{\mathcal{M}}(G(x))\cdot\sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))}
\end{align}
which, upon rearrangement, is the manifold change-of-variables formula.

Given a subset $A\subset \mathcal{M}$, we define its volume by,
\begin{align}
    \int_A ~\mathrm{dVol}(y) = \int_{G^{-1}(A)} \sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))}~\mathrm{d}x.
\end{align}
Such a definition of volume is sometimes called the ``surface measure'' and it is a generalization of arclength in the one-dimensional setting. Moreover, this notion of volume coincides with the $m$-dimensional Hausdorff area of $A$; this is a consequence of the {\it area formula} and a detailed discussion can be found in \citep{federer1969geometric}.



==> Manifold Density Estimation via Generalized Dequantization/appendices/son-elbo.tex <==
\clearpage
\section{Evidence Lower Bound for Special Orthogonal Group}\label{app:son-elbo}

Let $\mathbf{R}$ be a reflection matrix. Then using the fact that $\mathrm{O}(n) = \mathrm{SO}(n)\times\set{\mathrm{Id}_n, \mathbf{R}}$ we have,
\begin{align}
    \log \pi_{\mathrm{SO}(n)}(\mathbf{O}) &= \log \underset{\mathbf{S}\sim\mathrm{Unif}(\mathrm{Id}_n, \mathbf{R})}{\mathbb{E}} \pi_{\mathrm{O}(n)}(\mathbf{S}\mathbf{O}) + \log 2  \\
    &\geq \underset{\mathbf{S}\sim\mathrm{Unif}(\mathrm{Id}_n, \mathbf{R})}{\mathbb{E}} \log \pi_{\mathrm{O}(n)}(\mathbf{S}\mathbf{O}) + \log 2 \\
    &\geq \underset{\mathbf{S}\sim\mathrm{Unif}(\mathrm{Id}_n, \mathbf{R})}{\mathbb{E}}  \underset{\mathbf{L}\sim \tilde{\pi}_{\mathrm{Tri}_+}}{\mathbb{E}} \log \frac{\pi_{\R^{n\times n}}(\mathbf{S}\mathbf{O}\mathbf{P})}{\mathcal{J}(\mathbf{O}\mathbf{P})\cdot \tilde{\pi}_{\mathrm{Tri}_+}(\mathbf{L})} +  \log 2 \\
    &\geq \underset{\mathbf{S}\sim\mathrm{Unif}(\mathrm{Id}_n, \mathbf{R})}{\mathbb{E}}  \underset{\mathbf{L}\sim \tilde{\pi}_{\mathrm{Tri}_+}}{\mathbb{E}} \log \frac{\pi_{\R^{n\times n}}(\mathbf{S}\mathbf{O}\mathbf{P})}{\mathcal{J}(\mathbf{O}\mathbf{P})\cdot \tilde{\pi}_{\mathrm{Tri}_+}(\mathbf{L})}
\end{align}
where $\mathcal{J}(\mathbf{O}\mathbf{P}) \defeq \sqrt{\mathrm{det}((\nabla G(\mathbf{O}\mathbf{P}))^\top (\nabla G(\mathbf{O}\mathbf{P})))}$.

==> Manifold Density Estimation via Generalized Dequantization/appendices/stiefel-qr-decomposition.tex <==
\newpage
\section{Stiefel QR Decomposition}\label{app:stiefel-qr-decomposition}

In \cref{app:polar-decomposition-isomorphism} we discussed computing the positive definite component $\mathbf{P}$ as the principal square root of $\mathbf{A}^\top\mathbf{A}$. In our algorithm, $\mathbf{P}$ is represented according to its Cholesky factor, which is unique because $\mathbf{P}$ is (assuming $\mathbf{A}$ is full-rank). An alternative would be to compute a Cholesky factor of $\mathbf{A}^\top\mathbf{A}$ directly; such an approach allows us to use the QR decomposition in place of the polar decomposition.
\begin{proposition}
Suppose $\mathbf{A}\in \R^{m\times n}$ is a matrix of full-rank. The (unique) QR decomposition of $\mathbf{A}$ is
\begin{align}
    \mathbf{A} = \mathbf{Q}\mathbf{R}
\end{align}
where
\begin{align}
    \mathbf{L} &\defeq \mathrm{Cholesky}(\mathbf{A}^\top\mathbf{A}) \\
    \mathbf{R} &\defeq \mathbf{L}^\top \\
    \mathbf{Q} &\defeq \mathbf{A}\mathbf{R}^{-1}.
\end{align}
Moreover $\mathbf{Q}\in\mathrm{Stiefel}(m, n)$.
\end{proposition}
\begin{proof}
The uniqueness of $\mathbf{L}$ (and consequently $\mathbf{R}$) follows from the fact that the Cholesky decomposition of positive definite matrices is unique. Since $\mathbf{A}$ is of full-rank, $\mathbf{A}^\top\mathbf{A}$ is a positive definite matrix. Since $\mathbf{L}$ has positive diagonal entries, its determinant is non-zero and therefore has a unique inverse. This implies the uniqueness of $\mathbf{Q}$. The fact that $\mathbf{Q}$ is an element of the Stiefel manifold follows from direct evaluation:
\begin{align}
    \mathbf{Q}^\top\mathbf{Q} &= (\mathbf{R}^{-1})^\top \mathbf{A}^\top\mathbf{A} \mathbf{R}^{-1} \\
    &= \mathbf{L}^{-1} \mathbf{L}\mathbf{L}^\top(\mathbf{L}^\top)^{-1} \\
    &= \mathrm{Id}.
\end{align}
\end{proof}

\begin{proposition}
Let $(\mathbf{Q},\mathbf{L})\in\mathrm{Stiefel}(m,n) \times\mathrm{Tri}_+(n)$. The Jacobian determinant of the transformation $(\mathbf{Q},\mathbf{L})\mapsto \mathbf{Q}\mathbf{L}^\top$ is
\begin{align}
    \prod_{i=1}^n \mathbf{L}_{ii}^{m-i}.
\end{align}
\end{proposition}
\begin{proof}
See page 31 of \citep{edelman}.
\end{proof}


==> Manifold Density Estimation via Generalized Dequantization/appendices/torus-direct-dequantization.tex <==
\clearpage
\section{Torus Modulus Dequantization}\label{app:torus-modulus-dequantization}

Taking inspiration from \cref{app:integer-dequantization}, we turn now to consider another dequantization of the torus. To begin, identify the circle $\mathbb{S}^1$ with the interval $[0, 2\pi)$. We can construct a map from $\R$ to $\mathbb{Z}\times [0, 2\pi)$ by identifying $2\pi$-periodic points. Define the map $\tilde{G}(x) = (\lfloor x\rfloor, x~(\mod 2\pi))$. Let $\mathcal{O}_k = [2\pi k, 2\pi(k+1))$ for $k\in\mathbb{Z}$; on this interval we may define $G_k : \mathcal{O}_k \to \mathbb{Z}\times [0, 2\pi)$ by $G_k(x) = (k, x - 2\pi k)$ which satisfies $G \vert \mathcal{O}_k = G_k$. Because this map is nothing but a shift by $2\pi k$, it is invertible and volume preserving. Moreover, we may view $\mathbb{Z}\times[0, 2\pi)$ as a coordinate system for $\R$. Let $\pi_\R$ be a density on $\R$ and let $x\sim\pi_\R$. The associated density on $\mathbb{Z}\times [0, 2\pi)$ is therefore,
\begin{align}
    \pi_{\mathbb{Z} \times [0,2\pi)}(k, y) = \pi_{\R}(y + 2\pi k).
\end{align}
We may marginalize out the integers to obtain the density on $[0, 2\pi)$ as
\begin{align}
    \pi_{[0, 2\pi)}(y) = \sum_{k\in\mathbb{Z}}  \pi_{\R}(y + 2\pi k).
\end{align}

This idea is readily extended to higher dimensions. Because the torus is nothing but the product manifold of two circles, we may identify the torus with $[0,2\pi) \times[0, 2\pi)$. Let $\pi_{\R^{2}}$ be a density on $\R^2$ and let $G : \R^2\to \left[\mathbb{Z}\times[0, 2\pi)\right]^2$ be defined by $G(x_1, x_2) = (\tilde{G}(x_1), \tilde{G}(x_2))$. Following the precise reasoning from the one-dimensional case, if $x\sim\pi_{\R^2}$ then the density of $(x_1~(\mod 2\pi), x_2~(\mod 2\pi))$ is,
\begin{align}
    \pi_{[0, 2\pi)\times[0, 2\pi)}(y_1, y_2) = \sum_{k_1\in\mathbb{Z}} \sum_{k_2\in\mathbb{Z}} \pi_{\R^2}(y_1 + 2\pi k_1, y_2 + 2\pi k_2).
\end{align}

We call this approach {\it modulus dequantization}. This approach requires fewer dimensions than embedding the torus in $\R^{2m}$. In practice, the infinite sums over the integers may be approximated by truncating to a finite number of terms.

==> Manifold Density Estimation via Generalized Dequantization/appendices/universal-approximation-for-dequantized-density.tex <==
\clearpage
\section{Universal Approximation for the Dequantized Density}\label{app:universal-approximation-dequantized-density}

The purpose of this section is to give sufficient conditions on the dequantization of a distribution on a manifold into an ambient Euclidean space such that a suitably expressive normalizing flow on the Euclidean space could, in principle, learn the density to an arbitrary precision. The conclusion of this section is that it is sufficient that the distribution on the manifold and auxiliary structure be measurable with respect to the natural Borel $\sigma$-algebra and that the transformation between Euclidean space and the product space of the manifold and auxiliary structure be continuously differentiable. After stating this result, the remainder of the section is devoted to explaining what is meant by universal approximation of Euclidean densities.

\begin{definition}
Let $\mathcal{X}$ be a topological space. The smallest $\sigma$-algebra containing all the open sets of $\mathcal{X}$ is called the Borel $\sigma$-algebra. The Borel $\sigma$-algebra is denoted $\mathfrak{B}(\mathcal{X})$. An element $A\subset\mathfrak{B}(\mathcal{X})$ is called a Borel set.
\end{definition}
\begin{definition}
A measure $\mu$ on $\R^m$ is said to be absolutely continuous with respect to the Lebesgue measure if there exists a measurable function $\pi :\R^m\to\R_+$ such that
\begin{align}
    \mu(A) = \int_A \pi(x) ~\mathrm{d}x,
\end{align}
where $A\in\mathfrak{B}(\R^m)$.
\end{definition}
\begin{definition}
Let $\mathcal{X}$ and $\mathcal{Y}$ be topological spaces. A function $f:\mathcal{X}\to\mathcal{Y}$ is said to be Borel measurable if for all $E\in \mathfrak{B}(\mathcal{Y})$
\begin{align}
    f^{-1}(E) = \set{x \in \mathcal{X} : f(x)\in E} \in \mathfrak{B}(\mathcal{X}).
\end{align}
\end{definition}
\begin{proposition}\label{prop:measurable-compositions}
Let $f : \mathcal{X}\to\mathcal{Y}$ and $g : \mathcal{X}\to\mathcal{Y}$ be two Borel measurable functions. Then the product function $h(x) \defeq g(x) f(x)$ is also Borel measurable. Moreover, if $k:\mathcal{Y}\to\mathcal{Z}$ is another Borel measurable function then the composition $k\circ f:\mathcal{X}\to\mathcal{Z}$ is also Borel measurable.
\end{proposition}

\begin{proposition}\label{prop:measurable-density}
Let $U$ be an open subset of $\R^m$ and let $G:U\to \R^n$ be a homeomorphism on its image. Let $\mathcal{M}\defeq \set{G(x) : x\in U}$. Assume further that $G$ is a continuously differentiable function. Let $\mu_\mathcal{M}$ be a measure on $\mathcal{M}$ that is absolutely continuous with respect to the volume measure on $\mathcal{M}$; that is,
\begin{align}
    \mu_\mathcal{M}(A) = \int_A \pi_\mathcal{M}(y) ~\mathrm{dVol}(y)
\end{align}
where $\pi_\mathcal{M}:\mathcal{M}\to\R_+$ is a measurable function and $A\subset\mathcal{M}$ is a Borel subset. Then, if $y\sim \pi_\mathcal{M}$, the random variable $x\defeq G^{-1}(y)$ has a measurable density with respect the the Lebesgue measure given by
\begin{align}
    \pi_U(x) \defeq \pi_\mathcal{M}(G(x)) \cdot\sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))}.
\end{align}
\end{proposition}
\begin{proof}
By the manifold change-of-variables formula, the measure $\mu_\mathcal{M}$ is related to the Lebesgue measure on $\R^m$ according to,
\begin{align}
    \label{eq:manifold-measurable} \mu_\mathcal{M}(A) = \int_{G^{-1}(A)} \pi_\mathcal{M}(G(x)) \cdot\sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))} ~\mathrm{d}x.
\end{align}
Now we apply the results of \cref{prop:measurable-compositions} to show that the integrand on the right-hand side of \cref{eq:manifold-measurable} is a measurable function. Because $G$ is smooth it is continuous, and continuous functions are measurable. Therefore, when $A\in \mathfrak{B}(\mathcal{M})$ we obtain that $G^{-1}(A)\in\mathfrak{B}(U)$. Moreover, $\pi_\mathcal{M}\circ G$ is a measurable function with respect to the Borel $\sigma$-algebra on $U$ because the composition of measurable functions is measurable. Finally, since $G$ is continuously differentiable, and since the determinant and square-root are continuous functions, $\sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))}$ is also a measurable function.

Thus, if $y\sim \pi_\mathcal{M}$, the random variable $x\defeq G^{-1}(y)$ has a measurable density with respect the the Lebesgue measure given by
\begin{align}
    \pi_U(x) \defeq \pi_\mathcal{M}(G(x)) \cdot\sqrt{\mathrm{det}(\nabla G(x)^\top \nabla G(x))}.
\end{align}
\end{proof}
\begin{corollary}
The measure
\begin{align}
\mu_U(A) \defeq \int_A \pi_U(x)~\mathrm{d}x
\end{align}
is absolutely continuous with respect to the Lebesgue measure.
\end{corollary}


In the context of dequantization, we would like to understand the conditions under which the dequantization of a density on an embedded manifold $\mathcal{Y}$ via an auxiliary embedded manifold $\mathcal{Z}$ and a smooth, invertible function $G: U\to \mathcal{Y}\times\mathcal{Z}$ produces a Lebesgue measurable density on $U\subset\R^m$. 
\begin{proposition}\label{prop:dequantization-density}
Let $\mathcal{Y}$ and $\mathcal{Z}$ be embedded manifolds. Let $\pi_\mathcal{Y}$ be the density on $\mathcal{Y}$ defined with respect to the Riemannian volume element $\mathrm{dVol}_{\mathcal{Y}}$ and let $\pi_{\mathcal{Z}}(\cdot\vert y)$ be a density on $\mathcal{Z}$ (which may depend on $y\in \mathcal{Y}$) defined with respect to the Riemannian volume element $\mathrm{dVol}_{\mathcal{Z}}$. Suppose further that $\mathcal{Y}\times\mathcal{Z}=G(U)$, where $U$ is an open set of $\R^m$ and $G : U\to\mathcal{Y}\times\mathcal{Z}$ is continuously differentiable homeomorphism. If $(y,z)$ are random variables having density function $\pi_\mathcal{Y}(y)\pi_{\mathcal{Z}}(\cdot\vert y)$ with respect to the product element $\mathrm{dVol}_{\mathcal{Y}}\times\mathrm{dVol}_{\mathcal{Z}}$, then the random variable $x=G^{-1}(y, z)$ has a density with respect to Lebesgue measure if $\pi_\mathcal{Y}(y) \cdot \pi_\mathcal{Z}(z\vert y)$ is measurable with respect to $\mathfrak{B}(\mathcal{Y}\times\mathcal{Z}) = \mathfrak{B}(\mathcal{Y})\times\mathfrak{B}(\mathcal{Z})$.
\end{proposition}
\begin{proof}
This follows as a result of \cref{prop:measurable-density} when $\mathcal{M}=\mathcal{Y}\times\mathcal{Z}$ and $\mu_\mathcal{M}=\mu_{\mathcal{Y}\times\mathcal{Z}}$ is defined by
\begin{align}
    \mu_{\mathcal{Y}\times\mathcal{Z}}(A) = \int_{A} \pi_\mathcal{Y}(y) \cdot \pi_\mathcal{Z}(z\vert y) ~\mathrm{dVol}_{\mathcal{Z}}(z)~\mathrm{dVol}_{\mathcal{Y}}(y)
\end{align}
where $A\in\mathfrak{B}(\mathcal{Y}\times\mathcal{Z})$.
The conditions of the proposition are met because $U$ is an open subset of $\R^m$ by assumption and $G$ is a continuously differentiable homeomorphism by assumption. 
\end{proof}

% Let $\pi_\mathcal{Y}$ be the density on $\mathcal{Y}$ to be dequantized and let $\pi_{\mathcal{Z}}(\cdot\vert y)$ be a density on $\mathcal{Z}$, which may depend on $y\in \mathcal{Y}$. To apply \cref{prop:measurable-density}, identify $\mathcal{M}=\mathcal{Y}\times\mathcal{Z}$ and $\pi_\mathcal{M}(y, z) = \pi_\mathcal{Y}(y) \cdot \pi_\mathcal{Z}(z\vert y)$. \Cref{prop:measurable-density} therefore asserts that the probability distribution constructed in the Euclidean space by dequantization has a density with respect to Lebesgue measure when $\pi_\mathcal{Y}(y) \cdot \pi_\mathcal{Z}(z\vert y)$ is measurable with respect to $\mathfrak{B}(\mathcal{Y}\times\mathcal{Z}) = \mathfrak{B}(\mathcal{Y})\times\mathfrak{B}(\mathcal{Z})$ and $G: \R^m \to\mathcal{Y}\times\mathcal{Z}$ is continuously differentiable.

The importance of the open set $U$ is best seen through an example.
\begin{example}\label{ex:spherical-change-of-variables}
Let $U=\R^{3}\setminus\set{0}$ and consider the transformation $G : U\to\mathbb{S}^2\times\R_+$ by defined by
\begin{align}
    G(x) = (x / r, r).
\end{align}
where $r=\Vert x\Vert$. Thus, we see that $G$ is the spherical coordinate representation of the point $x\in U$. The inverse of $G$ is given by $G^{-1}(s, r) = rs$. Notice that by choosing $U$ to exclude the zero vector, we ensure that $G$ is indeed a homeomorphism; if the zero vector had not been included we would find that $G^{-1}(s, 0) = 0$ for all $s\in\mathbb{S}^2$ so that the inverse is not unique.

To see that $G$ is continuously differentiable, we compute
\begin{align}
    \frac{\partial r}{\partial x_j} &= \frac{x_j}{r} \\
    \frac{\partial}{\partial x_j} \paren{\frac{x_i}{r}} &= \frac{\delta_{ij}}{r} - \frac{x_ix_j}{r^3}
\end{align}
both of which are continuous for $x\in U$. Therefore, if $(r, s)$ is a random variable on $\mathbb{S}^2\times\R_+$ with Borel-measurable density, then the random variable $G^{-1}(r, s)$ has a density in $U$ with respect to Lebesgue measure by \cref{prop:dequantization-density}.
\end{example}


The existence of a Lebesgue measurable density in Euclidean space allows us to apply the theory of universal approximations of certain normalizing flows to guarantee that the dequantized distribution can be approximated arbitrarily well by a sufficiently expressive normalizing flow in Euclidean space.

The remaining discussion in this appendix is paraphrased from Section 3.4.3 in \citep{kobyzev2020normalizing}, which itself draws from \citep{pmlr-v97-jaini19a} and \citep{pmlr-v80-huang18d}. The essential idea is that one can produce auto-regressive normalizing flows whose couplings are dense in a space of functions that are guaranteed to have a universality property.

\begin{definition}
Let $T:\R^m\to\R^m$ be a function and write $T(x) = (T_1(x),\ldots, T_m(x))$ where $T_k : \R^m\to\R$. Such a function is called triangular if $T_k(x)$ depends only on $(x_1,\ldots, x_k)$
\end{definition}
\begin{definition}
Let $T:\R^m\to\R^m$ be a function and write $T(x) = (T_1(x),\ldots, T_m(x))$ where $T_k : \R^m\to\R$. Such a function is called increasing if $T_k$ is an increasing function of $x_k$.
\end{definition}
\begin{definition}\label{def:2021-05-05-auto-regressive}
An auto-regressive normalizing flow is a triangular map $(x_1,\ldots,x_m)\mapsto (y_1,\ldots,y_m)$ of the form
\begin{align}
    y_k = h(x_k\vert \Theta_k(x_1,\ldots,x_{k-1}))
\end{align}
where $h(\cdot\vert\theta) : \R\to\R$ is a bijection parameterized by $\theta\in \R^d$ and $\Theta_k :\R^{k-1}\to\R^d$ is a map that parameterizes $h$ according to $(x_1,\ldots,x_{k-1})$.
\end{definition}
In our experimentation on dequantization, we have {\it not} considered using auto-regressive flows in the ambient Euclidean space; neither RealNVP nor neural ODEs are auto-regressive in the sense of \cref{def:2021-05-05-auto-regressive}. Therefore, this discussion is primarily of theoretical interest.

\begin{definition}
Let $\mu$ be a probability measure on a measurable space $\mathcal{X}$ and let $x$ be a random variable taking values in $\mathcal{X}$. We say that the law of $x$ is $\mu$ if for all Borel sets $A\in\mathfrak{B}(\mathcal{X})$ we have
\begin{align}
    \mathrm{Pr}(x\in A) = \int_A ~\mathrm{d}\mu(x).
\end{align}
\end{definition}
The following result is from \citep{bogachev}.
\begin{proposition}\label{prop:2021-05-05-transport-map}
Let $\mu$ and $\mu'$ be probability measures that are absolutely continuous with respect to the Lebesgue measure. Let $x$ be a random variable whose law is $\mu$. Then there exists a triangular-increasing function $T$ such that the law of $T(x)$ is $\mu'$.
\end{proposition}
A construction of such a map in \cref{prop:2021-05-05-transport-map} is given by the Knothe-Rosenblatt rearrangement \citep{villani2008optimal}.

The following result is from \citep{pmlr-v80-huang18d}.
\begin{lemma}\label{lem:pointwise-convergence-map}
Let $\mu$ be a probability measure that is absolutely continuous with respect to Lebesgue measure. Let $T_n$ be a sequence of measurable maps converging pointwise to a map $T$. If the law of a random variable $x$ is $\mu$, then the random variables $T_n(x)$ converge in law to to the random variable $T(x)$.
\end{lemma}
% The proof follows from the application of the bounded convergence corollary of the dominated convergence theorem for probability spaces (which necessarily have finite measure).

The universality of auto-regressive normalizing flows can therefore be established by demonstrating that the functions $h$ appearing in \cref{def:2021-05-05-auto-regressive} are dense in the set of increasing monotone functions. One then applies \cref{prop:2021-05-05-transport-map,lem:pointwise-convergence-map} to demonstrate that any random variable $x$ with law $\mu$ can be transformed by an auto-regressive flow using the function $h$ into an approximation of a random variable $x'$ with law $\mu'$; the approximation has arbitrarily high fidelity as measured by convergence in law. See \citep{pmlr-v80-huang18d,pmlr-v97-jaini19a} for a discussion of parameterized families of functions $h$ that are known to possess this property.


In conclusion, \cref{prop:dequantization-density} gives the necessary conditions on product manifold densities and the change-of-variables $G$ to ensure the existence of a Lebesgue measurable density in an open subset of Euclidean space. We saw in \cref{ex:spherical-change-of-variables} how the choice of open set allows us to avoid pathological points in Euclidean space. Using the existence of the Lebesgue-measurable density, we may apply the theory of universal approximation of Lebesgue-measurable densities using auto-regressive normalizing flows to guarantee that the dequantized distribution can be approximated arbitrarily well. We note, however, that our experiments have not used auto-regressive normalizing flows.


% {\color{red}[
% There are a lot of loose ends as far as I can tell. 

% $G(U) \subset Y \times Z$ but doesn't mean that we cover all values of y. {\color{blue} $G(U) = Y\times Z$ by definition; this is line 747: let $M = ...$.} - That's a separate definition. In line 770 I say to identify $M = Y\times Z$. So, U is back to being a subset. And, nothing about getting rid of any pathological points in the context of what we're doing. Not clear. G is a homeomorphism on its image so there are no pathologies by definition.

% Ok. so the definition doesn't apply to QR decomposition and any of the ones we're using?

% I'm reading paragraph around 766. For all I can tell, this applies to any arbitrary set U. 

% I should have said open U to be consistent wirh prop 8.

% Yes, and still it wouls say any open subset of U. It doesn't say that G(U) = $Y \times Z$. It's clear if you already know it and already know the problem with pathological points, which isn't mentioned anywhere. It might be clear if the construction of what you're trying to do is stated, but the overall picture isn't stated. Usually, these things that are supposed to be clear are where holes in the proof show up. In this case, most likely, there could be some hole around the pathological points in the most general case, but they are kind of irrelevant to the construction that we actually use because the pahotlogical points are probably in nice places which are easy to characterize, but it might make the most general proof a little tricky. So it might mean that there would be some sort of leap of faith that we would phrase as a sketch of the proof. But maybe you can sort out all of it. For the sphere example, it's something about how we treat z=0, which we can exclude entirely by defining z>0 (there might still be a difficulty approaching 0, but I haven't thought it through), but you can of have to go and show how the constructions work with this argument, or what properties that constructions need to have.
% Most likely, these are not very interesting technical details, so we just need the big picture to be sufficiently clear that the reader can use the sketch to fill in the minimal gaps and we should leave unnecessary gaps that make life difficult for them unnecessarily.

% Can I call you. How about zoom actually?

% yes
% ok, but I can't go over all of it, you'll need to fix this and write it more clearly. 

% OK I thought it was clear from context of prop 8 but I can add it explicitly.

% Take spherical coordinates as an example. The open subset is $U = \R^3 \setminus\set{0}$ the product manifold is $Y\times Z= \mathbb{S}^{2} \times\R_+$. There are no pathologies by construction.

% The idea is that prop. 8 is fairly general statement that I'm going to apply to the product manifold $Y\times Z$. 


% Doesn't say that there is measure on $Y \times Z$ only where $G^{-1}((y,z)) \in U$ (otherwise not even defined). 

% {\color{blue} The measure on $Y\times Z$ is the Riemannian volume measure; equation 95.}

% Might also miss some measurability comments there, but likely negligible. Might require some statement about properties of $\pi_Z(z|y)$ but likely also not crucial.

% [Maybe? $G(U) \subset Y \times Z$ I think it need to be $G(R^m) = Y \times Z$ (but somehow exclude pathological points) and needs to further have some properties on $U$ where we actually care. ]

% Needs to tie everything together. What we claim that exists, (ideally, why we have these subsets that avoid pathologies+example), that this thing can be apprximated but autoregressive .... and reiterate that our specific implementation doesn't use autoregressive.
% ]}

==> Manifold Density Estimation via Generalized Dequantization/figures/dequantization-concept.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{images/dequantization.pdf}
    \caption{We show the case wherein $\mathcal{X}\cong\mathcal{Y}\times\mathcal{Z}$. Given a point $y\in \mathcal{Y}$, we consider the subspace $(y,\mathcal{Z})$ as the ``dequantization'' of $y$ into the product space $\mathcal{Y}\times\mathcal{Z}$. If $\mathcal{X}$ were equipped with a probability measure, then it would induce a probability measure on $\mathcal{Y}\times\mathcal{Z}$ via the pushforward measure (not shown). The probability measure on $\mathcal{Y}$ would then be obtained as the pushforward measure of the projection operator to $\mathcal{Y}$. If we suppose further that there is a density on $\mathcal{Y}\times\mathcal{Z}$ then we may obtain a formula for the density of the marginal distribution on $\mathcal{Y}$ via \cref{eq:marginal-density}.}
    \label{fig:dequantization}
\end{figure}

==> Manifold Density Estimation via Generalized Dequantization/figures/dequantization-roadmap.tex <==
\begin{figure*}[t!]
    \centering
    \scalebox{0.87}{
    \begin{tikzpicture}
    \node (A) at (0,0) {Spaces};
    \node (B) at (2,0) {$\R^m$};
    \node (change) at (3.9,0.5) {Change-of-Variables};
    \node (C) at (6,0) {$\mathcal{Y}\times\mathcal{Z}$};
    \node (D) at (10,0) {$\mathcal{Y}$};
    \path (B) -- node (cov) {$G$} (C);
    \path (C) -- node (quantization) {Quantization} (D);
    \draw[->] (B) --(cov)-- (C);
    
    \node (alpha) at (14,0) {$\mathcal{Y}\times\mathcal{Z}$};
    \path (D) -- node (dequantization) {Dequantization} (alpha);
    \draw[->] (D) --(dequantization)-- (alpha);
    
    \draw[->] (C) --(quantization)-- (D);
    \node (E) at (0,-2) {Densities};
    \node (F) at (2,-2) {$\pi_{\R^m}$};
    \node (G) at (6,-2) {$\pi_{\mathcal{Y}\times\mathcal{Z}}$};
    \node (H) at (10,-2) {$\pi_{\mathcal{Y}}$};
    \node (I) at (14,-2) {$\tilde{\pi}_{\mathcal{Z}}$};
    \node (J) [text width=2cm,align=center] at (14,-2.7) {Dequantization Density};
    \draw[->] (F) --(cov)-- (G);
    \draw[->] (G) --(quantization)-- (H);
    \node (impsamp) at (12,-2) {$\underset{z\sim\tilde{\pi}}{\mathbb{E}} \frac{\pi_{\mathcal{Y}\times\mathcal{Z}(\cdot, z)}}{\tilde{\pi}_{\mathcal{Z}}(z)}$};
    \draw[->] (I) --(impsamp)-- (H);
    \draw[->] (G) |- (J);
    \draw[->] (alpha) edge (I);
    
    \node (marginal) at (8.1,-1.5) {$\int_{\mathcal{Z}} \pi_{\mathcal{Y}\times\mathcal{Z}}(\cdot, z)~\mathrm{d}z$};
    
    \end{tikzpicture}}
    \caption{The dequantization roadmap. In the first row, we begin with $\R^m$.
    %(or a space identical to $\R^m$ up to a set of measure zero).
    This Euclidean space is transformed into the product of manifolds $\mathcal{Y}\times\mathcal{Z}$ via a change-of-variables $G:\R^m\to\mathcal{Y}\times\mathcal{Z}$. Quantization takes the product manifold $\mathcal{Y}\times\mathcal{Z}$ to its $\mathcal{Y}$-component alone. In the second row, we begin with a probability density $\pi_{\R^m}$ defined on $\R^m$. Under the change-of-variables $G$ we obtain a new probability density $\pi_{\mathcal{Y}\times\mathcal{Z}}$ which is related to $\pi_{\R^m}$ by the manifold change-of-variables \cref{eq:manifold-change-of-variables}. Quantizing $\mathcal{Y}\times\mathcal{Z}$ marginalizes out the $\mathcal{Z}$-component of $\pi_{\mathcal{Y}\times\mathcal{Z}}$. We similarly introduce a dequantization density $\tilde{\pi}_{\mathcal{Z}}$ and compute the marginal density on $\mathcal{Y}$ via importance sampling.}
    \label{fig:dequantization-roadmap}
\end{figure*}

==> Manifold Density Estimation via Generalized Dequantization/figures/dequantization-sphere-density.tex <==
% \begin{figure}[t!]
\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-1.5cm}
    \centering
    \includegraphics[width=0.4\textwidth]{images/dequantization-density.pdf}
    \caption{We model densities on a manifold as a projection, or ``quantization,'' onto the manifold from an ambient Euclidean space.  To enable density computations we use a ``dequantization density'' which can depend position on the manifold. In this figure the manifold in question is $\mathbb{S}^2$, embedded in $\R^3$ and the dequantization density, illustrated here for a set of locations along the equator of $\mathbb{S}^2$, is over $r\in \R_+$, the distance from the origin in the direction $y\in\mathbb{S}^2$. Density on the manifold can be estimated via importance sampling by marginalizing over $\R^+$ for a given $y\in\mathbb{S}^2$ using the dequantization distribution as an importance distribution.}
    \label{fig:dequantization-sphere-density}
\end{wrapfigure}

==> Manifold Density Estimation via Generalized Dequantization/figures/hyper-sphere-density.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hyper-sphere-approx-density-kl.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hyper-sphere-target-density-kl.png}
    \end{subfigure}
    \caption{Comparison of the density on $\mathbb{S}^3$ learned via RealNVP dequantization with a KL-divergence loss. We visualize $\mathbb{S}^2$-slices of $\mathbb{S}^3$ by examining the density when one of the hyperspherical coordinates is held fixed. The top set of slices shows the approximate density obtained via dequantization and the target density. The KL divergence is 0.01269 and the relative effective sample size is 97.70\%.}
    \label{fig:hyper-sphere-density}
\end{figure}

==> Manifold Density Estimation via Generalized Dequantization/figures/sphere-density.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/sphere-kl-approximation.png}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/sphere-target-density.png}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hyper-sphere-densities.png}
        \caption{}
    \end{subfigure}
    \caption{Figures (a) and (b): Comparison of the density on $\mathbb{S}^2$ learned via RealNVP dequantization with a KL-divergence loss estimated via importance sampling. The dequantization procedure is able to identify all modes of the density correctly. Figure (c): Comparison of the density on $\mathbb{S}^3$ learned via RealNVP dequantization with a KL-divergence loss. We visualize $\mathbb{S}^2$-slices of $\mathbb{S}^3$ by examining the density when one of the hyperspherical coordinates is held fixed. The top set of slices shows the approximate density obtained via dequantization and the target density. The KL divergence is 0.01269 and the relative effective sample size is 97.70\%.}
    \label{fig:sphere-density}
\end{figure}

==> Manifold Density Estimation via Generalized Dequantization/tables/elements.tex <==
\begin{table*}[h]
\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
Element                     & Notation                                        & Description                                                                                                                                                                                                             \\ \midrule
Ambient Euclidean Space     & $\mathcal{X}=\R^m$                              & Euclidean space in which the manifold of interest is embedded                                                                                                                                                           \\ 
Ambient Density             & $\pi_\mathcal{X}(\cdot\vert\theta)$             & A flexible family of densities parameterized by $\theta\in\R^{n_\mathrm{amb}}$ on $\mathcal{X}$                                                                                                                         \\
Change-of-Variables Mapping & $G: \mathcal{X}\to\mathcal{Y}\times\mathcal{Z}$ & \begin{tabular}[c]{@{}l@{}}A smooth mappingsatisfying the conditions of \cref{cor:partition-change-of-variables} or \cref{thm:manifold-change-of-variables} \\ where $\mathcal{Z}$ is an auxiliary manifold.\end{tabular}         \\
Dequantization Density      & $\tilde{\pi}_{\mathcal{Z}}(\cdot \vert \phi,y)$ & \begin{tabular}[c]{@{}l@{}}A non-vanishing family of dequantization distributions parameterized \\ by $\phi\in\R^{n_\mathrm{deq}}$ and possibly depending on $y\in\mathcal{Y}$.\end{tabular}                                                                       \\
Loss Function               & $\mathcal{L} : \R^{n_{\mathrm{amb}}\times n_{\mathrm{deq}}} \to \R$                                   & \begin{tabular}[c]{@{}l@{}}A loss function depending on $\set{y_1,\ldots, y_{n_\mathrm{obs}}}$, $\pi_\mathcal{X}$, and $\tilde{\pi}_{\mathcal{Z}}$ that\\  is differentiable in $\theta$ and $\phi$ and captures the quality of the density \\ estimate.\end{tabular} \\ \bottomrule
\end{tabular}
\caption{The five elements that we use to dequantize a manifold into an ambient Euclidean space using a change-of-variables and dequantization density for marginalization.}
\label{tab:elements}
\end{table*}

==> Manifold Density Estimation via Generalized Dequantization/tables/hypersphere-comparison.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison of dequantization to normalizing flows on the multimodal density on $\mathbb{S}^3$. Averages were computed using ten random trials for the dequantization procedures and nine random trials for the normalizing flow (one random trial exhibited divergent behavior and was excluded).}
    \vspace{1em}
    \scriptsize
    \begin{tabular}{l|rrrrr}
        Method & Mean MSE & Covariance MSE & $\mathrm{KL}(q \Vert p)$ & $\mathrm{KL}(p\Vert q)$ & Relative ESS \\ \bottomrule
Deq. ODE (ELBO) & 0.0009 $\pm$ 0.0001 & 0.0007 $\pm$ 0.0001 & 0.0072 $\pm$ 0.0002 & 0.0070 $\pm$ 0.0002 & 98.6490 $\pm$ 0.0388 \\
Deq. ODE (I.S.) & 0.0017 $\pm$ 0.0001 & 0.0022 $\pm$ 0.0002 & 0.0189 $\pm$ 0.0004 & 0.0180 $\pm$ 0.0004 & 96.6150 $\pm$ 0.0648 \\
Deq. RealNVP (ELBO) & 0.0003 $\pm$ 0.0001 & 0.0004 $\pm$ 0.0001 & 0.0384 $\pm$ 0.0010 & 0.0283 $\pm$ 0.0005 & 95.1880 $\pm$ 0.0771 \\
Deq. RealNVP (I.S.) & 0.0003 $\pm$ 0.0001 & 0.0003 $\pm$ 0.0000 & 0.0208 $\pm$ 0.0004 & 0.0180 $\pm$ 0.0004 & 96.6340 $\pm$ 0.0920 \\
Man. ODE & 0.0012 $\pm$ 0.0003 & 0.0008 $\pm$ 0.0002 & 0.0098 $\pm$ 0.0009 & 0.0094 $\pm$ 0.0007 & 98.1780 $\pm$ 0.1302 \\
M\"{o}bius & 0.0027 $\pm$ 0.0004 & 0.0014 $\pm$ 0.0003 & 0.0542 $\pm$ 0.0047 & --- & 88.7290 $\pm$ 0.9332 \\ 
\bottomrule
    \end{tabular}
    \label{tab:hyper-sphere-comparison}
\end{table*}

==> Manifold Density Estimation via Generalized Dequantization/tables/orthogonal.tex <==
\begin{table*}[t!]
    \centering
    \caption{Metrics of the dequantization algorithm in application to the orthogonal Procrustes problem and dequantization of a multimodal density on $\mathrm{SO}(3)$. When using the polar decomposition, results are averaged over ten independent trials for the multimodal distribution on $\mathrm{SO}(3)$ and nine independent trials for the orthogonal Procrustes problem; for the QR decomposition, results are averaged over nine trials.}
    \vspace{1em}
    \scriptsize
    \begin{tabular}{l|rrrrr}
        Experiment & Mean MSE & Covariance MSE & $\mathrm{KL}(q \Vert p)$ & $\mathrm{KL}(p\Vert q)$ & Relative ESS \\ \bottomrule
Procrustes (ELBO - Polar) & 0.0021 $\pm$ 0.0008 & 0.0012 $\pm$ 0.0005 & 0.0193 $\pm$ 0.0069 & 0.0173 $\pm$ 0.0053 & 96.9489 $\pm$ 0.7649 \\
Procrustes (I.S. - Polar) & 0.0038 $\pm$ 0.0020 & 0.0015 $\pm$ 0.0008 & 0.0301 $\pm$ 0.0126 & 0.0202 $\pm$ 0.0075 & 95.6944 $\pm$ 1.4654 \\
Procrustes (ELBO - QR) & 0.0011 $\pm$ 0.0003 & 0.0008 $\pm$ 0.0003 & 0.0124 $\pm$ 0.0032 & 0.0095 $\pm$ 0.0015 & 97.9678 $\pm$ 0.3325 \\
Procrustes (I.S. - QR) & 0.0015 $\pm$ 0.0005 & 0.0011 $\pm$ 0.0004 & 0.0174 $\pm$ 0.0072 & 0.0122 $\pm$ 0.0029 & 96.6267 $\pm$ 0.6326 \\ \midrule
$\mathrm{SO}(3)$ (ELBO - Polar) & 0.0007 $\pm$ 0.0002 & 0.0029 $\pm$ 0.0003 & 0.0443 $\pm$ 0.0011 & 0.0415 $\pm$ 0.0059 & 96.2930 $\pm$ 0.0649 \\
$\mathrm{SO}(3)$ (I.S. - Polar) & 0.0004 $\pm$ 0.0001 & 0.0014 $\pm$ 0.0001 & 0.0207 $\pm$ 0.0028 & 0.0235 $\pm$ 0.0029 & 97.7280 $\pm$ 0.1136 \\
$\mathrm{SO}(3)$ (ELBO - QR) & 0.0017 $\pm$ 0.0004 & 0.0054 $\pm$ 0.0006 & 0.0563 $\pm$ 0.0060 & 0.0363 $\pm$ 0.0041 & 93.5633 $\pm$ 2.1331 \\
$\mathrm{SO}(3)$ (I.S. - QR) & 0.0012 $\pm$ 0.0004 & 0.0020 $\pm$ 0.0004 & 0.0260 $\pm$ 0.0017 & 0.0219 $\pm$ 0.0021 & 94.3256 $\pm$ 2.8099 \\ \bottomrule
    \end{tabular}
    \label{tab:orthogonal-comparison}
\end{table*}

==> Manifold Density Estimation via Generalized Dequantization/tables/sphere-comparison.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison of dequantization to normalizing flows on the multimodal density on $\mathbb{S}^2$. Averages were computed using ten random trials for the dequantization procedures and eight random trials for the normalizing flow (because two random trials exhibited divergent behavior and were excluded). The dequantization procedure is illustrated for both the ELBO loss and the KL divergence loss.}
    \vspace{1em}
    \scriptsize
    \begin{tabular}{l|rrrrr}
        Method & Mean MSE & Covariance MSE & $\mathrm{KL}(q \Vert p)$ & $\mathrm{KL}(p\Vert q)$ & Relative ESS \\ \bottomrule
Deq. ODE (ELBO) & 0.0012 $\pm$ 0.0002 & 0.0006 $\pm$ 0.0001 & 0.0046 $\pm$ 0.0002 & 0.0046 $\pm$ 0.0002 & 99.0990 $\pm$ 0.0401 \\
Deq. ODE (I.S.) & 0.0014 $\pm$ 0.0002 & 0.0010 $\pm$ 0.0001 & 0.0029 $\pm$ 0.0001 & 0.0029 $\pm$ 0.0001 & 99.4170 $\pm$ 0.0225 \\
Deq RealNVP (ELBO) & 0.0004 $\pm$ 0.0001 & 0.0003 $\pm$ 0.0001 & 0.0231 $\pm$ 0.0010 & 0.0212 $\pm$ 0.0009 & 95.9540 $\pm$ 0.1688 \\
Deq. RealNVP (I.S.) & 0.0005 $\pm$ 0.0002 & 0.0002 $\pm$ 0.0000 & 0.0124 $\pm$ 0.0006 & 0.0115 $\pm$ 0.0006 & 97.8240 $\pm$ 0.1183 \\
Man. ODE & 0.0010 $\pm$ 0.0004 & 0.0009 $\pm$ 0.0002 & 0.0085 $\pm$ 0.0007 & 0.0083 $\pm$ 0.0007 & 98.3860 $\pm$ 0.1328 \\
M\"{o}bius & 0.0021 $\pm$ 0.0005 & 0.0019 $\pm$ 0.0005 & 0.0595 $\pm$ 0.0025 & --- & 89.2575 $\pm$ 0.4888 \\
\bottomrule
    \end{tabular}
    \label{tab:sphere-comparison}
\end{table*}

==> Manifold Density Estimation via Generalized Dequantization/tables/torus.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison of Deq. RealNVP to M\"{o}bius Flow flows on the multimodal density on $\mathbb{T}^2$. Averages were computed using ten random trials for the Deq. RealNVP procedures, direct, and M\"{o}bius Flow flow procedures.}
    \vspace{1em}
    \tiny
    \begin{tabular}{ll|rrrrr}
        Density & Method & Mean MSE & Covariance MSE & $\mathrm{KL}(q \Vert p)$ & $\mathrm{KL}(p\Vert q)$ & Relative ESS \\ \bottomrule
Correlated & Deq. RealNVP (ELBO) & 0.0019 $\pm$ 0.0007 & 0.0098 $\pm$ 0.0019 & 0.0072 $\pm$ 0.0005 & 0.0084 $\pm$ 0.0006 & 98.6510 $\pm$ 0.0958 \\
& Deq. RealNVP (I.S.) & 0.0024 $\pm$ 0.0007 & 0.0121 $\pm$ 0.0041 & 0.0038 $\pm$ 0.0004 & 0.0040 $\pm$ 0.0004 & 99.2570 $\pm$ 0.0796 \\
& Modulus & 0.0017 $\pm$ 0.0005 & 0.0072 $\pm$ 0.0021 & 0.0025 $\pm$ 0.0006 & 0.0025 $\pm$ 0.0006 & 99.5000 $\pm$ 0.1153 \\
& M\"{o}bius & 0.0004 $\pm$ 0.0002 & 0.0083 $\pm$ 0.0029 & 0.0021 $\pm$ 0.0002 & --- & 99.5850 $\pm$ 0.0332 \\ \midrule

Unimodal & Deq. RealNVP (ELBO) & 0.0010 $\pm$ 0.0003 & 0.0133 $\pm$ 0.0040 & 0.0066 $\pm$ 0.0004 & 0.0079 $\pm$ 0.0004 & 98.7240 $\pm$ 0.0761 \\
& Deq. RealNVP (I.S.) & 0.0011 $\pm$ 0.0003 & 0.0081 $\pm$ 0.0020 & 0.0021 $\pm$ 0.0002 & 0.0023 $\pm$ 0.0002 & 99.5980 $\pm$ 0.0317 \\
 & Modulus & 0.0014 $\pm$ 0.0003 & 0.0164 $\pm$ 0.0028 & 0.0028 $\pm$ 0.0003 & 0.0028 $\pm$ 0.0003 & 99.4340 $\pm$ 0.0531 \\
& M\"{o}bius & 0.0006 $\pm$ 0.0002 & 0.0055 $\pm$ 0.0037 & 0.0008 $\pm$ 0.0001 & --- & 99.8490 $\pm$ 0.0293 \\ \midrule

Multimodal & Deq. RealNVP (ELBO) & 0.0024 $\pm$ 0.0006 & 0.0158 $\pm$ 0.0026 & 0.0065 $\pm$ 0.0002 & 0.0075 $\pm$ 0.0002 & 98.7800 $\pm$ 0.0379 \\
& Deq. RealNVP (I.S.) & 0.0007 $\pm$ 0.0002 & 0.0061 $\pm$ 0.0014 & 0.0020 $\pm$ 0.0001 & 0.0022 $\pm$ 0.0002 & 99.6160 $\pm$ 0.0288 \\
& Modulus & 0.0016 $\pm$ 0.0007 & 0.0063 $\pm$ 0.0024 & 0.0035 $\pm$ 0.0004 & 0.0035 $\pm$ 0.0004 & 99.3030 $\pm$ 0.0725 \\
& M\"{o}bius & 0.0006 $\pm$ 0.0001 & 0.0070 $\pm$ 0.0039 & 0.0012 $\pm$ 0.0002 & --- & 99.7600 $\pm$ 0.0358 \\ \bottomrule
    \end{tabular}
    \label{tab:torus-comparison}
\end{table*}

==> figures/dequantization-concept.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{images/dequantization.pdf}
    \caption{We show the case wherein $\mathcal{X}\cong\mathcal{Y}\times\mathcal{Z}$. Given a point $y\in \mathcal{Y}$, we consider the subspace $(y,\mathcal{Z})$ as the ``dequantization'' of $y$ into the product space $\mathcal{Y}\times\mathcal{Z}$. If $\mathcal{X}$ were equipped with a probability measure, then it would induce a probability measure on $\mathcal{Y}\times\mathcal{Z}$ via the pushforward measure (not shown). The probability measure on $\mathcal{Y}$ would then be obtained as the pushforward measure of the projection operator to $\mathcal{Y}$. If we suppose further that there is a density on $\mathcal{Y}\times\mathcal{Z}$ then we may obtain a formula for the density of the marginal distribution on $\mathcal{Y}$ via \cref{eq:marginal-density}.}
    \label{fig:dequantization}
\end{figure}

==> figures/hyper-sphere-density.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hyper-sphere-approx-density-kl.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hyper-sphere-target-density-kl.png}
    \end{subfigure}
    \caption{Comparison of the density on $\mathbb{S}^3$ learned via RealNVP dequantization with a KL-divergence loss. We visualize $\mathbb{S}^2$-slices of $\mathbb{S}^3$ by examining the density when one of the hyperspherical coordinates is held fixed. The top set of slices shows the approximate density obtained via dequantization and the target density. The KL divergence is 0.01269 and the relative effective sample size is 97.70\%.}
    \label{fig:hyper-sphere-density}
\end{figure}
